3Dtrees.earth: community research infrastructure for tree and forest analysis using close-range LiDAR data

From individual trees to forest stands, three-dimensional structure shapes carbon, water, and energy flows, habitat conditions, and resource availability. Yet tree and forest structural attributes remain difficult to assess consistently across space and time. Close-range LiDAR (light detection and ranging) records detailed 3D structure from branches and trees to forest plots, including trees outside forests. However, broader reuse is constrained when data, acquisition context, processing, computation, and access conditions are maintained separately. We present 3Dtrees.earth, an operational community research infrastructure that brings close-range LiDAR datasets, analysis tools, and computing resources together while linking original observations to their metadata and processing outputs. As of 23 October 2026, the platform comprised 2,760 datasets, including 2,481 publicly visible datasets. These point cloud datasets span 46 countries on all six inhabited continents and include terrestrial, mobile, and uncrewed aerial laser scanning. Users can contribute and discover datasets, run standardized processing workflows on shared computing infrastructure, inspect point clouds and model predictions in the browser, and access data and processing outputs together with citation information. Workflows combine rule-based and machine-learning methods, with tools updated as methods advance. Outputs include raster products, individual-tree and semantic segmentation, and tree- and stand-level metrics. Original point clouds and processing records are retained, enabling reprocessing with improved tools while preserving provenance. With broader coverage, curation, and validation, this shared resource could extend individual surveys into a basis for model evaluation and benchmarking, cross-site synthesis, calibration and validation of larger-scale Earth observation products, and macroecological analysis.

==> figures/shared/figure2_style.tex <==

\definecolor{ftPlatform}{HTML}{FBE0EE}      %
\definecolor{ftPlatformCard}{HTML}{FDF0F7}  %
\definecolor{ftField}{HTML}{DFE6C8}         %
\definecolor{ftStandard}{HTML}{FDEAC9}      %
\definecolor{ftWorkflow}{HTML}{DFE6F2}      %
\definecolor{ftBlue}{HTML}{4F7FE3}
\definecolor{ftViolet}{HTML}{9A6FD6}
\definecolor{ftMagenta}{HTML}{E05AA6}
\definecolor{ftTeal}{HTML}{2BA59B}
\definecolor{ftOrange}{HTML}{EE9A3A}
\definecolor{ftPrep}{HTML}{8FA8DC}
\definecolor{ftGrey}{HTML}{8A919C}
\definecolor{ftInk}{HTML}{1A1A1A}
\definecolor{ftMuted}{HTML}{3C4656}
\definecolor{ftLine}{HTML}{6B7280}
\definecolor{ftCardEdge}{HTML}{E7CFDC}

\tikzset{
  ft/panel/.style={rounded corners=5pt, draw=none, inner sep=8pt},
  ft/card/.style={rounded corners=4pt, fill=white, draw=none, align=center,
    text=ftInk, inner xsep=6pt, inner ysep=5pt, font=\sffamily\footnotesize},
  ft/pill/.style={rounded corners=7pt, draw=none, text=white, align=center,
    inner xsep=7pt, inner ysep=3.5pt, minimum height=14pt,
    font=\sffamily\scriptsize\bfseries},
  ft/title/.style={font=\sffamily\small\bfseries, text=ftInk, inner sep=0pt},
  ft/sub/.style={font=\sffamily\scriptsize, text=ftMuted, inner sep=0pt, align=center},
  ft/arrow/.style={-{Latex[length=2mm]}, line width=0.8pt, draw=ftLine},
  ft/flow/.style={-{Latex[length=2mm]}, line width=0.9pt, dash pattern=on 3pt off 2pt},
  ft/planned/.style={-{Latex[length=2mm]}, line width=0.8pt, draw=ftLine,
    dash pattern=on 1.5pt off 1.5pt},
}

